Next generation proton PDFs with deuteron and nuclear uncertainties

As data become more precise, estimating theoretical uncertainties in global PDF determinations is likely to become increasingly necessary to obtain correspondingly precise PDFs. Here we present a next generation of global proton PDFs (NNPDF4.0) that include theoretical uncertainties due to the use of heavy nuclear and deuteron data in the fit. We estimate these uncertainties by comparing the values of the nuclear observables computed with the nuclear PDFs against those computed with proton PDFs. For heavy nuclear PDFs we use the nuclear nNNPDF2.0 set, while for deuteron PDFs we develop an iterative procedure to determine proton and deuteron PDFs simultaneously, each including the uncertainties in the other. Accounting for nuclear uncertainties resolves some of the tensions in the global fit of the proton PDFs, especially those between the nuclear data and the extended LHC data set used in NNPDF4.0.

==> tables/fits-unc.tex <==
\begin{table}[h]
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.13}
  \begin{tabularx}{0.8\textwidth}{lX}
    \toprule
    {\bf Fit label }     & { \bf Description }\\
    \midrule
    NNPDF4.0    & Baseline fit from NNPDF4.0 \\
    No nuclear unc. & Without nuclear uncertainties \\
    Heavy nuclear unc. & Heavy nuclear uncertainties only \\
    Heavy nuclear shifted & Heavy nuclear uncertainties with shifted central value \\
    Deuteron unc. & Deuteron uncertainties only \\
    Deuteron shifted & Deuteron uncertainties with shifted central value \\
    Shifted & (All) nuclear uncertainties with shifted central value \\  
    \bottomrule
  \end{tabularx}
  \caption{A summary of the fits with nuclear uncertainties.}
  \label{tab:fits-unc}
\end{table}


==> tables/fits.tex <==
\begin{table}[h]
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.13}
  \begin{tabularx}{\textwidth}{lllX}
    \toprule
    {\bf Iteration }  & {\bf Dataset }            & {\bf Fit ID }        & { \bf Description }\\
    \midrule
    Baseline    & Proton and Deuteron & global-base    & Same as {\tt base} fit in~\cite{Faura:2020oom}.\\
    \midrule
    Iteration 0 & Proton              & proton-ite0    & Same as baseline, but restricted to the proton dataset\\
    \midrule
    Iteration 1 & Deuteron            & deuteron-ite1  & Same as baseline, but restricted to the deuteron dataset
                                                         and supplemented with a proton covariance matrix determined
                                                         from the proton-ite0 fit according to
                                                         Eq.~\eqref{eq:protoncovmatrix}.\\
                & Proton and Deuteron & global-ite1-dw & Same as baseline, but supplemented with a deuteron covariance
                                                         matrix determined from the deuteron-ite1 fit according to
                                                         Eq.~\eqref{eq:deuteroncovmatrix}.\\
    \midrule
    Iteration 2 & Deuteron            & deuteron-ite2  & Same as deuteron-ite1, but with a proton covariance matrix
                                                         determined from the global-ite1-dw fit.\\
                & Proton and Deuteron & global-ite2-dw & Same as global-ite1-dw, but with a deuteron covariance matrix
                                                         determined from the deuteron-ite2 fit.\\
                & Proton and Deuteron & global-ite2-sh & Same as global-ite2-sh, but with a deuteron covariance matrix
                                                         and shifts determined according to
                                                         Eq.~\eqref{eq:deuteronshifted}.\\
    \bottomrule
  \end{tabularx}
  \caption{A summary of the fits performed in this study, see text for details.}
  \label{tab:fits}
\end{table}


==> tables/tab-chi2-deut.tex <==
%-------------------------------------------------------------------------------
\begin{table}[!t]
  \rowcolors{2}{gray!25}{white}
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.13}
  \begin{tabularx}{\textwidth}{lCCC}
    \toprule
    \rowcolor{gray!40}
    \textbf{Experiment}
    & \textbf{$N_{\rm dat}$}
    &\textbf{ deuteron-ite1}
    & \textbf{deuteron-ite2}\\
    \midrule
    SLAC  ($F_2^d$)
    &      34   &      0.81   &      0.84   \\
    BCDMS ($F_2^d$)
    &     248   &      1.02   &      1.04   \\
    NMC   ($F_2^d/F_2^p$)
    &     121   &      1.02   &      0.99   \\
    DYE866/NuSea ($\sigma_{pd}^{\rm DY}/\sigma_{pp}^{\rm DY}$)
    &      15   &      0.14   &      0.14   \\
    \midrule
    \rowcolor{gray!40}
    {\bf Total } & {\bf 418} & {\bf 0.97} & {\bf 0.98} \\
        \rowcolor{white}
    \bottomrule\\
  \end{tabularx}
  \caption{The values of the $\chi^2$ per data point for each dataset included
    in the fits of deuteron PDFs.}
  \label{tab:chi2-deut}
\end{table}
%-------------------------------------------------------------------------------


==> tables/tab-chi2-proton.tex <==
%-------------------------------------------------------------------------------
\begin{table}[!t]
  \rowcolors{2}{gray!25}{white}
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.13}
  \begin{tabularx}{\textwidth}{lCCCCC}
    \toprule 
    \rowcolor{gray!40}
    \textbf{Experiment}
    &  \textbf{$N_{\rm dat}$} &  \textbf{global-base} &  \textbf{global-ite1-dw} &  
    \textbf{global-ite2-dw} &  \textbf{global-ite2-sh} \\
    \midrule
    SLAC  ($F_2^d$)
    &         34 & 0.72 & 0.50 & 0.50 & 0.49 \\
    BCDMS ($F_2^d$)
    &        248 & 1.10 & 0.98 & 0.91 & 0.96 \\
    NMC   ($F_2^d/F_2^p$)
    &        121 & 1.00 & 0.79 & 0.78 & 0.82 \\
    DYE886/NuSea ($\sigma_{pd}^{\rm DY}/\sigma_{pp}^{\rm DY}$)
    &         15 & 0.47 & 0.53 & 0.71 & 1.06 \\
    \midrule
    SLAC  ($F_2^p$)
    &         33 & 0.88 & 0.93 & 0.91 & 0.91 \\
    BCDMS ($F_2^p$)
    &        333 & 1.30 & 1.30 & 1.29 & 1.30 \\
    NMC   ($F_2^p$)
    &        204 & 1.54 & 1.55 & 1.54 & 1.55 \\
    CHORUS
    &        832 & 1.15 & 1.14 & 1.14 & 1.14 \\
    NuTeV
    &         76 & 0.76 & 0.81 & 0.77 & 0.89 \\
    HERA I+II (incl.)
    &       1145 & 1.16 & 1.16 & 1.16 & 1.16 \\
    HERA ($\sigma_c^{\rm NC}$)
    &         37 & 1.42 & 1.43 & 1.43 & 1.44 \\
    HERA ($F_2^b$)
    &         29 & 1.11 & 1.11 & 1.11 & 1.11 \\
    DYE866/NuSea ($\sigma_{p}^{\rm DY}$)
    &         89 & 1.29 & 1.24 & 1.21 & 1.17 \\
    DYE605 ($\sigma_{p}^{\rm DY}$)
    &         85 & 1.11 & 1.10 & 1.09 & 1.12 \\
    CDF ($Z$ rap.)
    &         29 & 1.36 & 1.34 & 1.35 & 1.33 \\
    D0 ($Z$ rap.; $W$ asy.)
    &         45 & 1.18 & 1.15 & 1.16 & 1.17 \\
    ATLAS 
    &        211 & 1.13 & 1.12 & 1.12 & 1.10 \\
    \ \ \ ATLAS (Drell--Yan)
    &         75 & 1.44 & 1.40 & 1.41 & 1.35 \\
    \ \ \ ATLAS (jets)
    &         31 & 1.09 & 1.11 & 1.10 & 1.08 \\
    \ \ \ ATLAS ($Z p_T$)
    &         92 & 0.88 & 0.88 & 0.89 & 0.89 \\
    \ \ \ ATLAS (top)
    &         13 & 1.31 & 1.25 & 1.26 & 1.24 \\
    CMS 
    &        327 & 1.15 & 1.13 & 1.14 & 1.15 \\
    \ \ \ CMS (Drell--Yan)
    &        154 & 1.27 & 1.28 & 1.28 & 1.28 \\
    \ \ \ CMS (jets)
    &        133 & 0.99 & 0.93 & 0.97 & 1.05 \\
    \ \ \ CMS ($Z p_T$)
    &         28 & 1.32 & 1.30 & 1.31 & 1.31 \\
    \ \ \ CMS (top)
    &         12 & 0.88 & 0.87 & 0.89 & 0.87 \\
    LHCb
    &         85 & 1.62 & 1.59 & 1.67 & 1.66 \\
    \midrule
    \rowcolor{gray!40}
    {\bf Total } & {\bf 3978} & {\bf 1.18} & {\bf 1.16} & {\bf 1.16} & {\bf 1.16} \\
    \bottomrule\\
  \end{tabularx}
  \caption{The values of the $\chi^2$ per data point for each dataset included
    in the global fits of proton PDFs. The deuteron data are at the top of the table.}
  \label{tab:chi2-global}
\end{table}
%-------------------------------------------------------------------------------


==> tables/tab-fit-chi2.tex <==
\begin{table}[h]
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.13}
  \begin{tabularx}{\textwidth}{lllllllll}
    \toprule
    {\bf Fit }  & {\bf Total }   & BCDMS & SLAC & NMC & NuSea & E605 & NuTeV & CHORUS  \\
    \midrule
    No nuclear uncertainty & {\bf 1.265 } & 1.313 & 0.8217 & 1.658 & 0.8195 & 1.154 &  0.4569 & 1.165 \\
    \midrule
    Deuteron uncertainty & {\bf  1.251 } & 1.010 & 0.5425 & 0.8351 & 0.4227 & 1.182 & 0.4598 & 1.168 \\
    Deuteron shifted & {\bf 1.252 } & 1.056 & 0.5402 & 0.8451 & 0.5540 & 1.160 & 0.4563 & 1.164 \\
    \midrule
    Heavy nuclear uncertainty & {\bf 1.193} & 1.313 & 0.7650 & 0.8087 & 0.6739 & 0.4884 &  0.4641 & 0.9400 \\
    Heavy nuclear shifted & {\bf 1.211} & 1.319 & 0.7791 & 0.9858 & 0.6969 & 0.5021 &  0.4442 & 0.9621 \\
    \midrule
    Shifted & {\bf 1.187} & 1.018 & 0.5714 & 0.8481 & 0.3697 & 0.4935 & 0.4195  & 0.96205\\
    NNPDF4.0  & {\bf  1.174 } & 1.015 & 0.4972 & 0.8194 & 0.3971 & 0.4907 & 0.4602 & 0.9372 \\
    \bottomrule
  \end{tabularx}
  \caption{$\chi^2$ values for nuclear data sets for the various fits. \label{tab:nucfitchi2} }
  
\end{table}

